deltaBLEU: A Discriminative Metric for Generation Tasks with Intrinsically Diverse Targets

We introduce Discriminative BLEU (deltaBLEU), a novel metric for intrinsic evaluation of generated text in tasks that admit a diverse range of possible outputs. Reference strings are scored for quality by human raters on a scale of [-1, +1] to weight multi-reference BLEU. In tasks involving generation of conversational responses, deltaBLEU correlates reasonably with human judgments and outperforms sentence-level and IBM BLEU in terms of both Spearman's rho and Kendall's tau.

==> 10-relatedwork.tex <==
There have been several attempts to adapt \bleu to the needs of non-SMT tasks.
To foster diversity in paraphrase generation, Sun and Zhou ~\shortcite{DBLP:conf/acl/SunZ12} propose a metric termed i\bleu that deducts from the \bleu score of a candidate paraphrase, the inverse of the \bleu score computed between the source and paraphrase.
Their solution, in addition to being dependent on an adjustable parameter, is specific only to paraphrase.
For image captioning tasks, Vendantam et al.~\shortcite{VedantamZP14}, employ a variant of \bleu in which n-grams are weighted by tf-idf.
Neither of these modifications are particularly generalizable to evaluation of generated conversational responses.

